Prosody-Adaptable Audio Codecs for Zero-Shot Voice Conversion via In-Context Learning

Recent advances in discrete audio codecs have significantly improved speech representation modeling, while codec language models have enabled in-context learning for zero-shot speech synthesis. Inspired by this, we propose a voice conversion (VC) model within the VALLE-X framework, leveraging its strong in-context learning capabilities for speaker adaptation. To enhance prosody control, we introduce a prosody-aware audio codec encoder (PACE) module, which isolates and refines prosody from other sources, improving expressiveness and control. By integrating PACE into our VC model, we achieve greater flexibility in prosody manipulation while preserving speaker timbre. Experimental evaluation results demonstrate that our approach outperforms baseline VC systems in prosody preservation, timbre consistency, and overall naturalness, surpassing baseline VC systems.

==> sections/related.tex <==
\subsection{Zero-shot Voice Coversion}
The recent advancements in neural networks have significantly enhanced voice conversion (VC) technology \cite{DBLP:conf/iclr/PopovVGSKW22, DBLP:conf/icassp/LeeKLYY20, DBLP:conf/icassp/LianZY22}. Given the increasing demand for converting an input voice into an arbitrary target voice, zero-shot VC has become a focal point of interest. Traditionally, zero-shot VC has been achieved by disentangling semantic features (speech content) and acoustic features (speaker characteristics) from audio data. For instance, AutoVC \cite{DBLP:conf/icml/QianZCYH19} utilizes a bottleneck to manage the trade-off between speaker disentanglement and reconstruction quality. \cite{DBLP:conf/interspeech/ChouL19} introduced instance normalization (IN) to separate speaker and content representations. Other methods, such as the Disentangled Sequential Variational Autoencoder (DSVAE) \cite{DBLP:conf/icassp/LianZY22, DBLP:conf/interspeech/LianZA022}, have been developed to enhance disentanglement capabilities. \cite{DBLP:conf/iclr/YuanCZHGC21} minimized a sample-based mutual information upper bound between embeddings to decouple content and style information, while \cite{DBLP:conf/icassp/LiG0024} introduced a position-agnostic cross-attention mechanism for integrating style features from the reference speaker into semantic representations. LM-VC \cite{DBLP:journals/spl/WangCXTW23} employs a masked prefix language model to enhance content preservation and improve disentanglement.

While these disentanglement techniques facilitate training VC systems on non-parallel speech data, they still require high-fidelity audio \cite{DBLP:conf/interspeech/ZenDCZWJCW19, DBLP:conf/interspeech/KoizumiZKDYMB0H23}, which restricts scalability when applied to large datasets. Recent studies have sought to harness In-Context Learning (ICL) capabilities by training on extensive datasets, yielding impressive results in zero-shot text-to-speech (TTS) tasks \cite{zhang2023speak, wang2023neural, DBLP:conf/aaai/DuGSLLCWZ024, DBLP:conf/nips/LeVSKSMWMAMH23}. In this paper, we aim to extend these ICL capabilities from TTS to VC, developing a robust zero-shot VC system. 

\subsection{Prosody Control in Voice Conversion}
Prosody control has been a long-standing area of research, remaining essential due to its importance in controllable and emotional voice conversion. Prior work has explored various methods for encoding prosody information and disentangling it from content and timbre features. \cite{DBLP:conf/iscslp/LianZWLT21} proposed a convolution-based prosody encoder to effectively integrate prosody features into a baseline system. \cite{DBLP:conf/ijcnn/WangB22} introduced a prosody encoder using rank labels to learn disentangled prosody representations. \cite{DBLP:conf/icassp/ZhaoLSWKTM22} leveraged hybrid bottleneck features for extracting fine-grained and disentangled prosody characteristics, while PMVC \cite{DBLP:conf/mm/DengT0W0023} employed a contrastive-learning-based approach to separate content features from time-varying prosody features. 

In recent years, self-supervised pretrained models have also been used to disentangle semantic (content) features from acoustic features, such as prosody and timbre \cite{DBLP:conf/acl/HuangZWYTYLW0CS24, chen2024disentangling}. Building upon these developments, our work proposes a prosody control method for voice conversion by decomposing the audio codes generated by our backbone model, VALL-E X \cite{zhang2023speak}, into content, timbre, and prosody components. By leveraging ICL, our model attains strong zero-shot capability and offers precise control over prosody.




